Citance-Contextualized Summarization of Scientific Papers

Current approaches to automatic summarization of scientific papers generate informative summaries in the form of abstracts. However, abstracts are not intended to show the relationship between a paper and the references cited in it. We propose a new contextualized summarization approach that can generate an informative summary conditioned on a given sentence containing the citation of a reference (a so-called "citance"). This summary outlines the content of the cited paper relevant to the citation location. Thus, our approach extracts and models the citances of a paper, retrieves relevant passages from cited papers, and generates abstractive summaries tailored to each citance. We evaluate our approach using $\textbf{Webis-Context-SciSumm-2023}$, a new dataset containing 540K~computer science papers and 4.6M~citances therein.

==> table-evaluation-citance-primary.tex <==
\begin{table*}[th]
\small
\centering
\begin{tabular}{p{0.85\textwidth}}
\toprule
\textbf{DeepPavlov: Open-Source Library for Dialogue Systems} \\
\midrule
\noindent{\tt Citance Context} \\
\coloredbox{black!10}{Some of them are available for interactive online testing.}

\noindent \coloredbox{orange!10}{The skill implements Hybrid Code Networks (HCNs) described in (Williams et al., 2017).}

\noindent \coloredbox{black!10}{The model is configurable: embeddings, slot filling component and intent classifier can be switched on and off on demand.} \\ 
\midrule
\noindent \textbf{\ttfamily Abstract} \\
End-to-end learning of recurrent neural networks (RNNs) is an attractive solution for dialog systems; however, current techniques are data-intensive and require thousands of dialogs to learn simple behaviors. We introduce Hybrid Code Networks (HCNs), which combine an RNN with domain-specific knowledge encoded as software and system action templates. Compared to existing end-to-end approaches, HCNs considerably reduce the amount of training data required, while retaining the key benefit of inferring a latent representation of dialog state. In addition, HCNs can be optimized with supervised learning, reinforcement learning, or a mixture of both. HCNs attain state-of-the-art performance on the bAbI dialog dataset, and outperform two commercially deployed customer-facing dialog systems.\\ 

\noindent \textbf{\ttfamily GPT-citance-SciBert-top5}\\
After every dialogue, RL policy updates occur. State is maintained by both the RNN and the developer code. HCNs employ an RNN to gather dialogue state and select actions as well. In these structures, the RNN learns to handle entity values, such as storing them in memory. On the other hand, HCNs utilize an RNN that inherently deduces a state representation. \\ 

\noindent \textbf{\ttfamily GPT-similar-BM25-top2} \\
This paper introduces Hybrid Code Networks (HCNs), a model for end-to-end learning that combines learning an RNN with domain knowledge expressed via software and action templates. HCNs achieve the same performance as existing recurrent end-to-end techniques but with significantly less training data. The neural network can be trained with supervised learning or reinforcement learning by changing the gradient update applied. The model is applied to the bAbI dialog dataset and real customer support domains. HCNs can be optimized with reinforcement learning, using LSTM for the recurrent layer and the AdaDelta optimizer. \\ 

\noindent \textbf{\ttfamily LLaMA-CoT-citance-SciBert-top5} \\
The RL policy is updated after each dialogue. Both the RNN and the developer code retain state. HCNs also use an RNN to accumulate dialogue state and select actions. In each of these architectures, the RNN learns to manipulate entity values, for example by saving them in a memory. By contrast, HCNs use an RNN which automatically infers a representation of state. \\ 

\noindent \textbf{\ttfamily Vicuna-similar-BM25-top2} \\
This paper presents a new model called Hybrid Code Networks (HCNs) for end-to-end learning. HCNs allow developers to express domain knowledge and achieve better performance with less training data compared to existing techniques. The model is trained using supervised or reinforcement learning and can be applied to the bAbI dialog dataset and real customer support domains. The model can also be optimized with reinforcement learning.\\
\bottomrule
\end{tabular}
\caption{An example scenario where human annotators preferred the abstract over our summaries. Here, the citance clearly mentions the main contribution of the cited paper which is covered in more detail in the abstract. Contextualized summaries in this case  compared to the abstract. Here, we see that the citance itself is not descriptive of the main idea of the cited paper, hence requiring additional context for the reader to understand it. The abstract in this case is clearly insufficient.}
\label{tab:examples-summaries-main-idea}
\end{table*}

==> table-evaluation-citance-secondary.tex <==
\begin{table*}[th]
\small
\begin{tabular}{p{0.86\linewidth}}    
\toprule
\textbf{Semi-supervised sequence tagging with bidirectional language models} \\
\midrule
\noindent{\tt Citance Context} \\
\noindent \coloredbox{orange!10}{In both cases, we use the BIOES labeling scheme for the output tags, following previous work which showed it outperforms other options (e.g., Ratinov and Roth, 2009).}%

\noindent \coloredbox{black!10}{In addition to CNN-BIG-LSTM from Józefowicz et al. (2016), 1 we used the same corpus to train two additional language models with fewer parameters: forward LSTM-2048-512 and backward LSTM-2048-512. In all experiments, we fine tune the pre-trained Senna word embeddings but fix all weights in the pre-trained language models.}\\
\midrule
\noindent \textbf{\ttfamily Abstract} \\
We analyze some of the fundamental design challenges and misconceptions that underlie the development of an efficient and robust NER system. In particular, we address issues such as the representation of text chunks, the inference approach needed to combine local NER decisions, the sources of prior knowledge and how to use them within an NER system. In the process of comparing several solutions to these challenges we reach some surprising conclusions, as well as develop an NER system that achieves 90.8 F1 score on the CoNLL-2003 NER shared task, the best reported result for this dataset.\\ \vspace{0.1cm}

\noindent \textbf{\ttfamily GPT-citance-SciBert-top5} \\
In order to achieve the most accurate comparison, we provided each system with unprocessed text and relied on the system's ability to split sentences and tokenize them. This approach divides the Viterbi decision process into separate maximization tasks over smaller segments, where a greedy strategy is effective. Perceptron-based systems have demonstrated competitiveness in Named Entity Recognition (NER) and text chunking (Kazama and Torisawa, 2007b; Punyakanok and Roth, 2001; Carreras et al., 2003). We defined the model and its features using the LBJ (Rizzolo and Roth, 2007) modeling language. It is important to note that in this experiment, we also utilized token-level accuracy on the CoNLL dataset. The BILOU scheme proposes learning classifiers that can identify the Beginning, Inside, and Last tokens of multi-token chunks, as well as Unit-length chunks. \\ 

\noindent \textbf{\ttfamily GPT-similar-BM25-top2} \\
We analyze some of the fundamental design challenges and misconceptions that underlie the development of an efficient and robust NER system. In particular, we address issues such as the representation of text chunks, the inference approach needed to combine local NER decisions, the sources of prior knowledge and how to use them within an NER system. In the process of comparing several solutions to these challenges we reach some surprising conclusions, as well as develop an NER system that achieves 90.8 F1 score on the CoNLL-2003 NER shared task, the best reported result for this dataset. \\ \vspace{0.1cm}

\noindent \textbf{\ttfamily LLaMA-CoT-citance-SciBert-top5} \\
For the most accurate comparison, we have presented each system with raw text, and relied on the system's sentence splitter and tokenizer. This separation breaks the Viterbi decision process into independent maximization of assignment over short chunks, where the greedy policy performs well. Systems based on perceptron have been shown to be competitive in NER and text chunking (Kazama and Torisawa, 2007b; Punyakanok and Roth, 2001; Carreras et al., 2003). We specify the model and the features with the LBJ (Rizzolo and Roth, 2007) modeling language. Also note that in this experiment we have used token-level accuracy on the CoNLL dataset as well. The BILOU scheme suggests to learn classifiers that identify the Beginning, the Inside and the Last tokens of multi-token chunks as well as Unit-length chunks. \\ 

\noindent \textbf{\ttfamily Vicuna-similar-BM25-top2} \\
A simple technique of using word clusters generated from unlabeled text can improve performance of dependency parsing, Chinese word segmentation, and NER. The technique is based on word class models and uses a binary tree to represent words. The approach is related to distributional similarity, but not identical. The system's performance is significantly impacted by the choice of encoding scheme, and the less used BILOU formalism outperforms the widely adopted BIO tagging scheme. \\
\bottomrule

\end{tabular}
\caption{An example scenario where human annotators preferred our summaries compared to the abstract. Here, we see that the citance itself is not descriptive of the main idea of the cited paper, hence requiring additional context for the reader to understand it. The abstract in this case is clearly insufficient.}
\label{tab:examples-summaries-side-idea}
\end{table*}


==> table-query-variants-and-ir-models.tex <==
\begin{table}[ht!]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lp{0.6\columnwidth}}
\toprule
\textbf{Retrieval Setting} & \textbf{Description} \\
\midrule
\textbf{\tt CQ-BM25} & Citance used as the query, documents ranked with BM25. \\
\textbf{\tt CQ-SciBERT} & Citance used as the query, documents ranked based on cosine similarity of SciBERT embeddings. \\
\textbf{\tt CQ-KW-BM25} & Keywords extracted from citance used individually as queries, documents ranked with BM25. Ranked lists are then fused into a final ranking. \\
\textbf{\tt CQ-KW-SciBERT} & Keywords extracted from citance used individually as queries, documents ranked based on cosine similarity of SciBERT embeddings. \\
\textbf{\tt NQ-BM25} & Citance and surrounding sentences (i.e., the \emph{neighbors} context) used as the query, documents ranked with BM25. \\
\textbf{\tt NQ-SciBERT} & The \emph{neighbors} context used as the query, documents ranked based on cosine similarity of SciBERT embeddings. \\
\textbf{\tt NQ-KW-BM25} & Keywords extracted from the \emph{neighbors} context used individually as queries, documents ranked with BM25. Ranked lists are then fused into a final ranking. \\
\textbf{\tt NQ-KW-SciBERT} & Keywords extracted from the \emph{neighbors} context used individually as queries, documents ranked based on cosine similarity of SciBERT embeddings. Ranked lists are then fused into a final ranking. \\
\textbf{\tt SQ-BM25} & Citance and two semantically similar sentences in the same paragraph (i.e., the \emph{similar} context) used as the query, documents ranked with BM25. \\
\textbf{\tt SQ-SciBERT} & The \emph{similar} context used as the query, documents ranked based on cosine similarity of SciBERT embeddings.  \\
\textbf{\tt SQ-KW-BM25} & Keywords extracted from the \emph{similar} context used individually as queries, documents ranked with BM25. Ranked lists are then fused into a final ranking. \\
\textbf{\tt SQ-KW-SciBERT} & Keywords extracted from the \emph{similar} context used individually as queries, documents ranked based on cosine similarity of SciBERT embeddings. Ranked lists are then fused into a final ranking. \\
\bottomrule
\end{tabular}
\caption{Overview of the various retrieval settings to find relevant content from the cited paper. Documents may be sentences or paragraphs. For the keyword-based settings, the final ranking is obtained by a weighted aggregation of the rankings based on the cosine similarity of a keyword and the citance. }
\label{tab:retrieval-settings}
\end{table}

==> table-retrieval-scenarios.tex <==
\begin{table}[ht!]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lp{0.45\columnwidth}}
\toprule
\textbf{Scenario} & \textbf{(Query, Retrieval Model)} \\
\midrule
\textbf{\tt citance-BM25} & (citance, BM25)\\
\textbf{\tt citance-SciBERT} & (citance, cosine similarity) \\
\textbf{\tt citance-keywords-BM25} & (keywords from citance, BM25)  \\
\textbf{\tt citance-keywords-SciBERT} & (keywords from citance, cosine similarity) \\
\textbf{\tt neighbors-BM25} & (citance and its neighbors, BM25) \\
\textbf{\tt neighbors-SciBERT} & (citance and its neighbors, cosine similarity) \\
\textbf{\tt neighbors-keywords-BM25} & (keywords from citance and its neighbors, BM25) \\
\textbf{\tt neighbors-keywords-SciBERT} & (keywords from citance and its neighbors, cosine similarity) \\
\textbf{\tt similar-BM25} & (citance and two similar sentences, BM25) \\
\textbf{\tt similar-SciBERT} & (citance and two similar sentences, cosine similarity) \\
\textbf{\tt similar-KW-BM25} & (keywords from citance and two similar sentences, BM25) \\
\textbf{\tt similar-KW-SciBERT} & (keywords from citance and two similar sentences, cosine similarity) \\
\bottomrule
\end{tabular}
\caption{Overview of the 12 retrieval scenarios to fetch relevant content (sentences or paragraphs) from the cited paper. For the keyword-based scenarios, first, each keyword is used as a query to rank the documents. Next, a final ranking is obtained by the weighted aggregation of the individual rankings based on the cosine similarity of a keyword and the citance.}
\label{tab:retrieval-scenarios}
\end{table}
